On Designing a Two-stage Auction for Online Advertising

For the scalability of industrial online advertising systems, a two-stage auction architecture is widely used to enable efficient ad allocation on a large set of corpus within a limited response time. The current deployed two-stage ad auction usually retrieves an ad subset by a coarse ad quality metric in a pre-auction stage, and then determines the auction outcome by a refined metric in the subsequent stage. However, this simple and greedy solution suffers from serious performance degradation, as it regards the decision in each stage separately, leading to an improper ad selection metric for the pre-auction stage. In this work, we explicitly investigate the relation between the coarse and refined ad quality metrics, and design a two-stage ad auction by taking the decision interaction between the two stages into account. We decouple the design of the two-stage auction by solving a stochastic subset selection problem in the pre-auction stage and conducting a general second price (GSP) auction in the second stage. We demonstrate that this decouple still preserves the incentive compatibility of the auction mechanism. As the proposed formulation of the pre-auction stage is an NP-hard problem, we propose a scalable approximation solution by defining a new subset selection metric, namely Pre-Auction Score (PAS). Experiment results on both public and industrial dataset demonstrate the significant improvement on social welfare and revenue of the proposed two-stage ad auction, than the intuitive greedy two-stage auction and other baselines.

==> 21fupa_main_wsdm/21fupa_old_doc.tex <==

% optimization problem: general objective
    % computing power to support the feature
     
    \section{Introduction}

    % 研究问题是电商的广告拍卖：为了匹配广告和用户，决策使用的是拍卖  
    
    Our research problem in this work comes from the multi-stage cascade decision system \cite{wang2020cold} in a large scale online display advertising system on an e-commerce platform. 
    This online advertising system serves billions of users and millions of advertisers every day by matching the advertisements of goods to its interested users. The advertising system decides the matching through an auction in each page view request from every user. 
    % 拍卖的结果由 bid 和 pctr 共同决定
    The auction process decides allocation of the $K$ ad positions on the page and the corresponding payment the allocated advertiser should pay to the advertising system. The two essential factors, allocation and payment, are determined by the advertiser's valuation of a click on her advertiser, i.e. the $bid$, and also by the probability that the user clicks on the ad which reflects the user's interests towards the ad, i.e. the predicted click through rate $pctr$. 
    % 拍卖机制  
    The allocation rule and payment rule consists of the auction mechanism. For the instance of the most widely used auction mechanism in online advertising, generalized second price auction (GSP) \cite{edelman2007internet}, the allocation rule is ranking the ads by $bid \times pctr$ and then matching the top $K$ ads the corresponding $K$ ad positions on the page, while the payment rule charges the rank $k<K$ ad the lowest bid she needs to still win the $k$-th ad position. 
    
    % 拍卖机制需要 IC【什么时候提这件事，后面再提】  
    Even with a clear defined procedure, auction mechanisms differ from traditional algorithms because the $bid$'s input to a auction mechanism come from rational advertisers who may strategically misreport their valuation for their own benefit, e.g. to use less money but obtain better ad position. Therefore, the auction mechanism should be incentive compatible \cite{nisan2007algorithmic}, i.e. to motivate the bidders reporting their true valuations.
    
    % 为了广告主用户广告平台的三方利益，拍卖的广告候选集很大，好处是
    % （1）对于广告主和用户，使得高效的匹配可能性更大，更好满足用户购物需求和广告主的营销目标  
    
    To maximize the efficiency of the marketing, the candidate set to the auction process is typically large. The mainly purpose of using a large candidate set is to optimize the efficiency of matching between user and ads. For the advertisers and users, a larger size of candidate ad set means more chance of efficient matching between ads and users that satisfy users' shopping demand and advertisers' marketing goal at the same time.
    % （2）[这似乎未必成立，先不写，evaluation 或者 discussion 再写，和 proposition 1 之间的关系] 对于广告系统，可以增加竞争机会和使得竞争更加激烈，从而获得更多广告收入  
    For the advertising system, a larger candidate set not only provides the advertisers with more competition opportunities in the long run, but also encourages a more sufficient competition among the advertisers, which finally results in a higher advertising revenue \cite{bulow1994auctions}. 
    
    % 但是为了用户体验，必须要在有限时延和算力下处理大的候选集  
    However, to ensure a smooth user experience, the system should finish above auction process in a strict latency limitation using a constrained computation resource \cite{jiang2020dcaf}.
    % 因为拍卖的分配和付费的逻辑都比较简单，系统吞吐量的瓶颈主要来自预估  
    While the computation of allocation rule and payment rule is simple, the bottle neck of the throughput of the advertising system is at the prediction module of $pctr$.
    % 为了精准的预估，模型使用神经网络在复杂的特征上面进行在线推理
    For an accuracy online prediction of the $pctr$, the system use sophisticated neural networks which inference the $pctr$ based on rich features from the user and the ad. On the one hand, thus a heavy model can not predict $pctr$ for every ad in the large candidate set in limited latency; on the other hand, as system depends heavily on the $pctr$ to make decision, there will be loss of optimization performance if the system only depends on the $pctr$ from a fast but inaccurate prediction module.
    
    % 为了让系统在有限时间和算力上达到尽可能高的优化表现，采用两层架构  
    To enable a high optimization performance in limited response latency, the auction system follows a two-stage cascade architecture. 
    % 第一阶段是 pre-allocation，使用 coarse pctr  
    In the early stage, called pre-allocation stage, a light weighted fast prediction module output coarse $\hat{pctr}$'s and the decision module ranks by $\hat{pctr}\cdot bid$. 
    % 第二阶段是 formal auction
    The top $M$ ads to in pre-allocation enters the next stage, called regular auction stage, where the heavy slow but accurate prediction module computes $pctr$ for the $M$ ads, and then auction mechanism works based on $pctr\cdot bid$ to decide the allocation and payments of $K$ ad positions.
    
    % 两个模型有两点不同  
    The light and heavy prediction model differ in two aspects: (1) the amount of information in the input features and (2) the complexity and representation ability in model structure. 
    
    % 这种不同使得两个模型有无法消除的性能差距 
    Due to the differences, there are inevitable performance gap between the light and heavy models. The gap causes that a high quality ad with the top $K$ $pctr \cdot bid$ value is filtered in the pre-allocation stage. Then this ad loses a fairly proper exposure chance, and also the advertising system suffers some loss in social welfare.
    
    \begin{figure}[h]
      \centering
      \includegraphics[width=\linewidth]{./21fupa_main_wsdm/fig/architecture.pdf}
      \caption{Architecture of two-stage auction system. }
      \Description{}
      \label{fig:architecture}
    \end{figure}
    
    \subsection{Prediction then Decision Cascade System}
    % 这个问题和场景广泛存在  
    In fact, the two-stage advertising auction system is a concrete instance of multi-stage \emph{prediction then decision} cascade system, a common seen architecture for latency and performance tradeoff in large scale online service.
    
    % 为什么需要有预估和决策两个模块分开  
    % 1. 预估模块的通用性，可以适用于各种决策的链路  
    % 2. 决策的可解释性  
    % 3. 预估不应该受到决策的影响  
    In each stage, there are separate prediction and decision modules. One may argue that the separability of prediction and decision mainly results in the loss of decision performance. We agree on that in some scenarios like learning to rank in recommender system, the deep integration of prediction of a user interest towards documents and the decision of ranking on the documents outperforms the separate prediction and ranking paradigm. However, in some scenarios, like the online advertising auction, the separability of prediction and decision is important. The main reasons are: (1) The decision relies on not only the prediction results, but also other factors from strategic input source, like the bid from the advertiser. To ensure the stability and long term healthy evolution of the system, the decision process should be incentive compatible, i.e. encouraging truthful report. (2) The decision rule should be interpretable, understandable and convincing to the participants. For example, an advertiser can easily understand from the formula $pctr \cdot bid$ that a higher $pctr$ means a more interested user and if she values much to a user's click, reporting a high $bid$ increases her chance to win the exposure. (3) The prediction module can work as service for all decision scenario, only if the prediction works for a general objective which is not directly affected by various of downstream decision modules.
    
    % 我们分析了这种架构中预估模块和决策模块的特点  
    
    Now, we summarize the general characteristics of the multi-stage prediction then decision cascade architecture.
    \begin{itemize}
      \item For the prediction modules, all of them serves a common prediction task. The ones in the earlier stage use less data features and output coarser prediction with simple neural networks, but are faster and have higher throughput, while the ones in the later stage use more data features and output finer prediction with sophisticated neural networks, but are slower and with lower throughput.
      \item For the decision modules, the earlier ones handle larger candidate sets, but there are larger decision redundancy because many outputs in this stage make no difference to the final results of the system, while the later ones handle smaller candidate sets, but there are little decision redundancy.
    \end{itemize}
    
    % 有工作尽可能提高预估模块的性能  
    There have been some works discussing how to improve the decision performance of multi-stage prediction then decision cascade architecture by narrowing the accuracy gap between the light and heavy model. 
    % 但是我们从另一个角度进行考虑，去改造决策模块  
    In this work, we improve the whole system decision performance by designing the early decision module. 
    The main idea is to leverage (1) the relationship between the prediction modules caused by the information structure of their input, and (2) the larger decision redundancy in the early stage.
    
    
    \subsection{Pre-allocation Optimization}
    % 现在回到具体的 pre-allocation 场景  
    For a clear representation, hereafter we turn back from the general multi-stage prediction then decision cascade architecture to our concrete scenario of pre-allocation in the two-stage advertising auction system. 
    
    We summarize our contributions here.
    % 首先我们把如何设计 pre-allocation decision 去最大化 sw 和 topk acc 建模为 scp  
    First, we model the problem of design a new decision module in pre-allocation stage which maximizes the expected social welfare as a stochastic combinatorial programming.
    
    % 然后我们分析了传统的实现为什么损失了性能
    Second, based on this modeling, we show that the canonical implementation of pre-allocation which simply ranking by $\hat{pctr}\cdot bid$ losses efficiency. 
    Specifically, we formalize relationship between the prediction output by two prediction modules in the same system, by leveraging that both prediction modules works on the same prediction task and trained with the data samples generated from the same whole system, and the heavy prediction module has additional features than the light prediction module. 
    
    % 然后我们为两个任务分别设计了近似的打分函数和确切的打分函数
    Third, we reduce our optimization problem to the NP-hard set cover. 
    Then we propose a practical learning based method named Pre-Allocation Decision (PAD) as an approximate solution. 
    Specifically, we propose loss functions from two views of social welfare optimization and a close problem of top $K$ accuracy optimization, based on probabilistic model and principle of maximum likelihood estimation.
    
    Finally, in empirical evaluation on real-world industrial data, we show that PAD methods demonstrate highly positive effect on social welfare, and also on metrics according user experience and ad platform revenue. 
    
    % TODO contribution
    
    \section{System Model}
    
    % 总分
    % 一 我们先介绍记号来表示我们的两阶段拍卖系统  
    % 二 我们介绍最大化社会福利的优化目标
    % 三 我们分析了预估模块和真实点击之间的信息差距，然后得到 利用最好预估进行决策 的原则
    % 四 我们将 pre allocation 决策问题定义为 scp  
    In this section, we first describe the notations to illustrate the two-stage auction system model. Second, we introduce the efficiency optimization objective of the auction system. Third, we analyze the information hierarchy among the two prediction modules and the true click behavior of the user, then we lead to the principle of leveraging the best prediction module in decision. Finally, we propose the formation of designing a pre-allocation decision module as a stochastic combinatorial programming.
    % ====
    
    % 我们正式描述两阶段的拍卖系统如下  
    % 一次页面展示广告请求中，拍卖系统收到的初始集合。  
    % 调用轻量预估模块，预估模块使用特征 z  
    % 然后 pre-allocation 根据信息 x 决策选出 M 候选集合。
    % x 信息包含了高度融合的预估值和广告的基本信息，比如 bid  
    % bid 是广告主报告的对于用户点击一次广告的估值
    
    \subsection{Basic Notations}
    
    We formally describe the two-stage cascade auction system here. 
    In every page view request, the pre-allocation stage receives an initial candidate ad set $\sx_N$, which contains $N$ ads, from upstream matching server who selects the set $\sx_N$ from the total ad sets by analyzing the user's shopping interests. 
    The light prediction module in pre-allocation system stage, denoted as $\M_L$, predicts the coarse $\hat{pctr}_i$ for every ad $i$ from $\sx_N$, with a light neural network using ad and user feature $z_i$.
    Then, pre-allocation decision module selects $M$ ads to form the subset $\sx_M\subset \sx_N$, using information $x_i$ for ad $i\in\sx_N$. Here, $x_i$ contains the highly integrated prediction results, e.g. $\hat{pctr}$ from the light prediction module, and other a few basic ad information, such as $bid$s for ads $i$.
    $bid_i$ is the advertiser's valuation of the user clicking on ad $i$. 
    
    % 接着 M 候选集被送到正式拍卖阶段  
    % 正式拍卖阶段重新进行更精确的预估，使用更加复杂的特征和网络  
    % 最后进行 GSP ，pctr * bid 计算分配和扣费 
    
    Then, the selected $\sx_M$ is passed to formal auction stage.
    The heavy prediction module in formal auction stage, denoted as $\M_H$, predicts the fine $pctr_i$ for each ad $i\in\sx_M$, with a sophisticated neural network using more ad and user feature $(z_i,\tilde{z}_i)$.
    Finally, the decision module in formal auction stage allocates $K$ ad positions and decides the corresponding payment by running a general second price (GSP) auction: allocates the $k$-th best ad position on the page to the ad $i(k)$ who has the $k$-th highest $pctr_{i(k)}\cdot bid_{i(k)}$, and its corresponding payment is $pctr_{i(k+1)}\cdot bid_{i(k+1)}/pctr_{i(k)}$.
    
    % ====
    
    % 广告拍卖系统的优化目标  
    % 作为一个广告拍卖系统，他的终极优化目的之一是高效匹配广告和消费者。
    % 每当被展示出得广告 i(k) in SK 被用户点击，相应的广告主就获得了 bid i 的点击营销价值，同时用户的点击行为也意味着广告符合了他的购物兴趣  
    % 【接下来是随机变量进行表达】
    % 然而在拍卖阶段，用户的点击行为并未发生，只能够建模为一个服从 伯努利 分布的随机变量 CLK  
    % 因此点击营销价值也是随机变量 Vi = CLK * bid ，分布和期望是 
    % 我们假设 CLK 独立，则 V 也独立。 
    % 于是广告系统的高效匹配目标可以定义为 期望点击社会福利，即展示集合的期望点击价值之和  
    
    \subsection{Efficiency optimization in ad auction}
    
    One of the ultimate goal of online advertising auction system is to efficiently match the ads and the user.
    Every time when a user clicks on an ad $i(k)\sx_K$ on his web page, the corresponding advertiser will obtain a marketing value of $bid_{i(k)}$ for this interaction with the user. At the same time, this click from the user represents that this ad exposure fits his shopping interesting. The higher the sum of click values, the system achieves more efficiency.
     
    However, during the auction process before ad exposure, we can only model the user's click behavior to ad $i$ as a random variable sampled from Bernoulli distribution, $\clk_i\sim Ber(c_i)$, where $\Pr[\clk_i=1]=c_i$.
    Also, the click marketing value is also a random variable $V_i=\clk_i\cdot v_i$, that $\Pr[V_i=v_i]=c_i$, $\Pr[V_i=0]=1-c_i,$ and $\E[V_i]=c_i\cdot v_i$.
    We assume the user clicks among the ads in a page view are independent, i.e. any subset of $\{\clk_i\}_{i\in\sx_N}$ are independent. 
    Then, given $(v_1,...,v_N)$, any subset of $\{V_i\}_{i\in\sx_N}$ are also independent.
    
    The ultimate goal of efficiency optimization in ad auction system can be achieved by selecting the exposure set $\sx_K\in\sx_N$ that maximizes the expected click social welfare, i.e. the sum of expected click marketing value,
    $$\max_{\sx_K} \quad \E_{V}[\sum_{i\in \sx_K} V_i].$$
    
    % ====
    
    % 跟随最好的预估模型  
    % 常用的处理方法是对点击事件的伯努利分布的参数进行统计学习的估计  
    % 预估模块估计的点击率是利用统计学习的方法估计伯努利分布的参数  
    % 这就是链路中的预估模型做的事情，使用用户和广告的特征预测点击的概率  
    % 然而无论是简单的还是复杂的预估模块输入的特征都只是真实世界中所有决定点击发生的一信息的一个子集  
    % 设相对于 z tilde z 之外的所有和点击行为相关的隐藏信息是 zh，则点击事件在给定了 z tilde z 和 zh 之后是定值  
    % 我们证明基于不同的信息决策 top K 的话，会出现获得的 social welfare 的 hierarchical gap  
    
    \subsection{Leverage the best prediction module}
    
    The practical and widely adopted approach for maximizing the above expected clicked social welfare is to estimate the parameter $c_i$ for Bernoulli distribution $\clk_i\sim Ber(c_i)$ via statistical learning. 
    This is exactly what the prediction modules in this two-stage systems do, i.e. use ad and user features to predict the probability of click.
    However, no matter how advanced and sophisticated our prediction module be, its input features are only a true subset of all correlated information in the world that finally determines the user's click or non-click behavior.
    Let $z_i^h$ be all the hidden information, in addition to $z_i,\tilde{z}_i$, that are correlated to the user's click behaviors, then the indicator $\mathbf{1}[\clk_i=1|z_i,\tilde{z}_i,z_i^h]$ evaluates to a deterministic value. 
    We show the hierarchical gap among the expected clicked social welfare induced by choosing top $K$ from $N$ ads under different amount of information.
    
    \begin{equation}
    \label{eq:hierarchical-gap}
      \begin{aligned}
        & \E_{\{(z_i,\tilde{z}_i,z_i^h)\}_i^N} 
        [ \mathtt{SumTopK}(\{v_i\cdot \mathbf{1}[\clk_i=1|z_i,\tilde{z}_i,z_i^h]\}) ] \\
      = & \E_{\{(z_i,\tilde{z}_i)_i^N\}}
        [ \sum_{z_i^h}\mathtt{SumTopK}(\{v_i\cdot \mathbf{1}[\clk_i=1|z_i,\tilde{z}_i,z_i^h]\}) \Pr[z_i^h|z_i,\tilde{z}_i]] \\
      \geq & \E_{\{(z_i,\tilde{z}_i)_i^N\}}
        [ \mathtt{SumTopK}(\{v_i\cdot \Pr[\clk_i=1|z_i,\tilde{z}_i]\}) ] \\
      \geq & \E_{\{z_i\}_i^N} 
        [ \mathtt{SumTopK}(\{v_i\cdot \Pr[\clk_i=1|z_i]\}) ]. \\
      \end{aligned}
    \end{equation}
    
    % 推导中的变换都基于假设：给定了 zi 之后 CLKi 互相间独立
    % SumTopK 是一个 n 维空间中的函数，表示【】
    % 注意 SumTopK 是定义域上面的凸函数  
    % 第一个大于等于是因为【】
    % 第二个大于等于和第一个是相似的原因  
    The transform in Eq.\ref{eq:hierarchical-gap} are all based on the assumption that $\{\clk_i\}_i^N$ are independent given $\{z_i\}_i^N$. 
    $\mathtt{SumTopK}:\mathbb{R}^n \rightarrow \mathbb{R}$, $n\geq K$ is a function which sums up the $K$ largest elements in a $n$-dim vector of size $n\geq K$. 
    Note that $\mathtt{SumTopK}$ is a convex function in $\mathbb{R}^n$.
    The first inequality is due to that 
    $$\mathbf{1}[\clk_i=1|z_i,\tilde{z}_i,z_i^h]\Pr[z_i^h|z_i,\tilde{z}_i]=\Pr[\clk_i=1|z_i,\tilde{z}_i],$$
    and Jensen's inequality along with the convexity of $\mathtt{SumTopK}$. 
    The reason for the second inequality is similar to the first one. 
    
    % 这个 hierarchical gap 的公式展示一个直观的结论，使用更多的信息作出的决策不会比使用更少的信息差
    % 下面假设预估模块基于给定的特征输出的点击率就是真实点击行为分布中具有同样特征的条件分布下的伯努利分布参数，pctr(z)=Pr[clki=1|z]  
    % 则可以得到两个约等于式子
    Eq.\ref{eq:hierarchical-gap} shows an intuitive results that we can make no worse decision if we use more related information. 
    Now we assume that the predicted click through rate from the prediction modules are sufficiently aligned with the Bernoulli parameters of corresponding conditional distribution given the feature, 
    i.e. $\hat{pctr}_i(z_i)$ from the light prediction module and $pctr_i(z_i,\tilde{z}_i)$ from the heavy prediction module are good estimations of the $\hat{c}_i(z_i)=\Pr[\clk_i=1|z_i]$ and $c_i(z_i,\tilde{z}_i)=\Pr[\clk_i=1|z_i,\tilde{z}_i]$, respectively.
    Now we have 
    $$\begin{aligned}
    & \E_{\{(z_i,\tilde{z}_i)_i^N\}}
    [ \mathtt{SumTopK}(\{v_i\cdot \Pr[\clk_i=1|z_i,\tilde{z}_i]\}) ] \\
    \approx & \E_{\{(z_i,\tilde{z}_i)_i^N\}} [\mathtt{SumTopK}(\{v_i\cdot pctr(z_i,\tilde{z}_i)\}) ],
    \end{aligned}$$
    $$\begin{aligned}
    & \E_{\{z_i\}_i^N} 
    [ \mathtt{SumTopK}(\{v_i\cdot \Pr[\clk_i=1|z_i]\}) ] \\
    \approx & \E_{\{z_i\}_i^N} 
    [ \mathtt{SumTopK}(\{v_i\cdot \hat{pctr}(z_i)\}) ]. \\
    \end{aligned}$$
    % 注意 SumTopK 可以看作计算 GSP 拍卖中的 expected clicked social welfare 
    % 由最后两个大于等于，如果我们暂时忽略掉两阶段的架构，最大化 GSP sw 的方法是使用最好的预估模型
    Note that $\mathtt{SumTopK}(\{v_i\cdot pctr_i\})$ is the expected clicked social welfare under GSP auction. 
    Therefore, by the last two lines of Eq.\ref{eq:hierarchical-gap}, if we temporarily ignore the two-stage auction architecture, and focus on choosing $K$ ads from the initial $N$ candidate ads, the best way for maximizing expected clicked social welfare in GSP is to use $pctr$s from the prediction module who can effectively use the most correlated features, i.e. $\M_H$ in our auction system.
    
    % ====
    
    \subsection{Optimization Problem of Pre-allocation}
    
    % 由于算力限制，没法在短时间内对 N 个广告都使用好模型进行 pctr 预测  
    % 为了解决这个问题，系统进行了时间和表现上的权衡，在 pre allocation stage 使用 light prediction module 然后在 formal stage 使用高级模型  
    
    Due to the limitation of computational resources, the system can not afford the workload of estimating $pctr$ for all $N$ ads using the heavy and slow $M_H$ during the limited latency of online service.
    Therefore, the system makes tradeoff between time and performance by firstly selecting a middle subset $\sx_M$ with the $\hat{pctr}$ from the light but fast prediction module $\M_L$ in pre-allocation stage, and secondly running GSP auction on $\sx_M$ with $pctr$ from the heavy but accurate prediction module $\M_H$ in formal auction stage. 
    
    % 在这样提升了吞吐量的同时，系统却面临了表现损失的风险
    % 如果 M 集合选中了最好的 K 个，那么这 K 个最终会在正式拍卖中胜出，就不会有性能的损失
    % 但是如果 M 集合漏掉了最好的 K 个，那么就有表现的损失  
    % 因此由前面提到的利用最好的预估模型的原则，pre allocation 应该尽可能使得选出的 M 集合覆盖 fine pctr * bid 大的广告
    % 同时，由于在正式拍卖使用 GSP，只有 M 集合中最大的 K 个会被展出，所以实际上我们只需要使得 M 集合的前 K 的 fine pctr * bid 之和尽可能大
    While this two-stage system improves online throughput, it is also at risk of suffering loss in optimization of click social welfare.
    If the pre-allocation stage chooses a middle subset $\sx_M$ that fully covers the $K$ ads with the top $pctr\cdot bid$, then during the formal auction stage, then during the formal auction stage, these $K$ top ads will finally win the exposure, hence no loss of expected clicked social welfare.
    However, if any ad $i(k)$ with a top $K$ $pctr\cdot bid$ is filtered out in pre-allocation stage, then the displayed sets differs from the optimal top $K$ set, and the system suffers a loss of expected clicked social welfare compared to using heavy prediction model $\M_H$ only.  
    Therefore, by the principle of leveraging the best prediction module, the decision module in pre allocation should make $\sx_M$ cover as much ads with high $pctr \cdot bid$ as possible. Besides, as only the ads with top $K$ $pctr\cdot bid$ in $\sx_M$ will be displayed after running the GSP auction, the pre-allocation decision module should  make the sum of top $K$ $pctr\cdot bid$ in $\sx_M$ as large as possible.
    
    % 我们形式化得到设计 pre-allcoation decision module 去选择一个子集去服务于最大化整个系统的点击社会福利的优化问题：一个随机组合规划
    % 【】
    % 注意我们复用一下 SumTopK 的符号，来在这里表示集合函数  
    % 这里的下标表示了 【】
    Therefore, we formalize the problem of designing a pre-allocation decision module which selects a subset $\sx\subset \sx_N$ to serve for maximizing the expected clicked social welfare of the two-stage auction system as below stochastic combinatorial programming (SCP),
    \begin{equation}
    \label{eq:opt-problem-set-form}
      \begin{array}{r@{\quad}r@{\quad}l}
        (SCP) & \max_{\sx_M(x)} & \E_{\{(x,pctr)\}_i^N} 
                [\stk(\{\sx_M(x), x, pctr\})] \\
              & s.t. & |\sx_M(x)| = M
      \end{array}.
    \end{equation}
    Recall that $x$ is the input information to pre-allocation decision module which includes $bid$, the output from the light prediction module $\M_L$ such as $\hat{pctr}$, and a few other ad related features, for each $i\in\sx_N$. 
    Note that we abuse the notation $\stk$ a little that 
    \begin{equation}
    \label{eq:func-sumtopk}
      \stk(\{\sx, x, pctr\})=\sum_{j=1}^K bid_{i(j)} pctr_{i(j)},
    \end{equation}
    where $\sx$ represents a set function mapping a subset of $\sx_N$ with the corresponding $pctr_i\cdot bid_i$ for each $i\in\sx_N$.
    The subscript $i(j)$ means ranking the ads by their $pctr_i\cdot bid_i$, \ie,
    $$pctr_{i(1)} \cdot bid_{i(1)} \geq \ldots \geq pctr_{i(N)} \cdot bid_{i(N)}.$$
    
    % From Proposition \ref{prop:gsp-max-csw}, 
    % we know that for any set $\sx_M$, the auction stage will maximize expected click social welfare by displaying the $K$ ads with the largest $c_i\cdot v_i$ from $\sx_M$. Therefore, with fixed auction mechanism GSP in auction stage of the two-stage system, the problem of maximizing expected clicked social welfare is reduced to maximizing the sum of top $K$ values from set $\sx_M$, i.e. to select a set $\sx_M$ which maximizes the sum of top $K$ values of $\{c_i\cdot v_i\}_{i\in \sx_M}$.
    
    % However, as the predicted click through rate $c_i$ is unknown for the pre-allocation module. From the Bayesian view, there is a random variable $C_i$ representing the unknown predicted click-through rate in the pre-allocation stage, and then if the ad $i$ is passed to the auction stage, the process that real time prediction module computes the $c_i$ can by seen as sampling from the distribution of $C_i$. 
    % We define a set of random variables $\{W_i\}_{i\in \sx_N}$ that $W_i=C_i\cdot v_i$, whose realization is $w_i=c_i\cdot v_i$ when the factor variable $C_i$ is realized as $c_i$. 
    % Thus, to serving the system's ultimate objective of maximizing click social welfare, the optimization problem of pre-allocation is intuitively reduced to select a subset $\sx_M$ of $M$ random variable $W_i$ from $\sx_N$ that maximizes the sum of top $K$ realized $w_i$. This is a stochastic combinatorial optimization problem. We presents the formulation as below.
    
    % 定义集合函数 SumTopK
    % First, we define a set function $\mathtt{SumTopK}:2^n\rightarrow\mathbb{R}^*$, over any set of cardinality $n\geq K$,
    
    % ====
    
    \section{A Tentative Solution}
    
    % 总分 TODO
    % 我们在这里介绍一种最为直接的预分配的决策模块  
    % 通过分析它所处的系统中的两个预估模型之间的关系，我们得到他的
    % 
    % 根据粗排打分以及粗排面向精排校准来选到底是哪里不好  
    
    In this section, we first discuss a canonical solution of pre-allocation decision module. We analysis the intrinsic principles behind the solution and show its limitation on performance by connecting it to a degenerated version of the \emph{SCP} problem.
    
    % 1. tentative solution of pre-allocation
    % - coarse prediction vs pctr
    % - inefficiency of the pre-allocation
    
    As the system cannot afford the computation of predict click through rate with the sophisticated but heavy model $\mathtt{M}_H$ for all $N$ ads, a canonical solution of pre-allocation stage is to build a fast and light-weighted version model $\mathtt{M}_L$ to predict a coarse predicted click through rate $\hat{c}_i$ for each ad $i\in\sx_N$. 
    Both the heavy and light version models, $\mathtt{M}_H$ and $\mathtt{M}_L$, aims at predicting the click through rate, i.e. the probability that the user clicks the ad. The problem of predicting click through rate is defined as a binary classification, with two types of labels, \emph{click=1} and \emph{click=0}, which means the user click and not click the ad, respectively. 
    % 把这种架构定义为 TENTATIVE
    We describe an solution called \emph{TENTATIVE} which leverages $\mathtt{M}_L$ and $\mathtt{M}_H$.
    \begin{definition}
      \emph{TENTATIVE}: (1) $\mathtt{M}_L$ predicts the coarse click through rate $\hat{c}_i$ of each ad in the large set $\sx_N$; (2) the $M$ ads with the highest $\hat{c}_i\cdot v_i$ are selected to form set $\sx_M$; (3) $\mathtt{M}_H$ predicts the click through rate $c_i$ of each ad in $\sx_M$; (4) GSP auction ranks the $M$ ads by $c_i\cdot v_i$ and display the $K$ top ads.
    \end{definition} 
    
    % 举出实际系统中这种实现的具体体现
    Due to the limited latency, the light model $\mathtt{M}_L$ uses simpler input features than the heavy model $\mathtt{M}_H$. Denote the input feature to the light model as \emph{light feature} $z$. The heavy model not only has access to \emph{light feature} $z$ but also to \emph{additional feature} $\tilde{z}$.
    To illustrate, we compare a typical light model \emph{COLD} \cite{wang2020cold} and two typical heavy models \emph{DIN} \cite{zhou2018deep} and \emph{DIEN} \cite{zhou2019deep}. Both models have access to the basic user profile which include the age, gender, \emph{etc} and the basic target ad feature consists of corresponding goods id, shop id, category id, and \emph{etc}. The differences in two models' input features mainly comes from two parts. (1) User behavior data: the heavy model \emph{DIN} input historical user behaviors in recent several weeks for adaptively activating the user's interests with the target ad, while the light model \emph{COLD} simply uses cross features of the user and the target ad as a compact representation of user's interests. (2) Cross features: the heavy model \emph{CAN} uses rich cross features of ad such as Cartesian products of category id and goods id, while the light model uses few ad cross features.
    
    % 两个模型在训练样本上的关系
    \subsection{Relation between $\mathtt{M}_L$ and $\mathtt{M}_H$}
    
    As both models differ on input features, their output predictions also varies. In Proposition \ref{prop:two-ctr-relation}, we show the relation between the output predictions from two models in a simple scenario.
    
    \begin{proposition}
    \label{prop:two-ctr-relation}
      If $\mathtt{M}_L$ and $\mathtt{M}_H$ are training on the same set of data samples $D=\{(z_j, \tilde{z}_j, y_j)\}_{j\leq|D|}$. For any data sample $j$, $z_j\in\Gamma$ is the light feature for both light and heavy model, while $\tilde{z}_j\in\tilde{\Gamma}$ is the additional feature for heavy model only. $y_j\in\{0,1\}$ is the label. Both $\mathtt{M}_L$ and $\mathtt{M}_H$ are trained on training set $D$ to minimize cross entropy loss function 
    \begin{equation}
    \label{eq:loss-ce}
      \begin{aligned}
        & \min_{\hat{c}(z)} \quad -\sum_{j\in|D|} y_j \log \hat{c}(z_j) + (1-y_j) \log (1-\hat{c}(z_j)), \\
        & \min_{c(z,\tilde{z})} \quad -\sum_{j\in|D|} y_j \log c(z_j,\tilde{z}_j) + (1-y_j) \log (1-c(z_j,\tilde{z}_j)).
      \end{aligned}
    \end{equation}
    Then the prediction functions $\hat{c}(z)$ for $\mathtt{M}_L$ and $c(z,\tilde{z})$ for $\mathtt{M}_H$ satisfies that
    \begin{equation}
    \label{eq:dctr-vs-pctr}
      \forall z \in \Gamma, \quad
      \hat{c}(z) = \sum_{\tilde{z}\in\tilde{\Gamma}} c(z,\tilde{z}) \Pr[\tilde{z}|z].
    \end{equation}
    \end{proposition}
    
    % 这个 prop 现在的缺陷 
    % 只能够在 离散的 \Gamma 和 \tilde{\Gamma} 并且已经完全在训练数据中出现过的情况中使用。
    % 这里由于直接限制了真实的数据集，所以我们直接就是 empirical risk optimization ，而不用考虑采样的分布  
    \begin{proof}
      Denote total training data sample set as $D=\bigcup_{(z,\tilde{z})} (D^+(z,\tilde{z})\cup D^-(z,\tilde{z}))$, 
      where $D^+(z,\tilde{z})=\{(z,\tilde{z},y)|y=1\}$ and $D^-(z,\tilde{z})=\{(z,\tilde{z},y)|y=0\}$, as the positive and negative training data samples set respectively, for each $(z,\tilde{z})\in \Gamma\times \tilde{\Gamma}$. 
      $D^+(z)=\bigcup_{\tilde{z}} D^+(z,\tilde{z})$ and $D^-=\bigcup_{\tilde{z}} D^-(z,\tilde{z})$ represent the positive and negative training data samples set respectively, for each $z\in\Gamma$.
      Then, the model $\hat{c}(z)$ and $c(z,\tilde{z})$ trained on the sample set $D$, which aims at minimizing the cross entropy loss, maximizes
      \begin{equation}
      \label{eq:amgm}
        \begin{aligned}
        & \sum_{z\in\Gamma} |D^+(z)| \cdot \log \hat{c}(z) + 
          \sum_{z\in\Gamma} |D^-(z)| \cdot \log (1-\hat{c}(z)) \\
        = & \log \prod_{z\in\Gamma} \hat{c}(z)^{|D^+(z)|}(1-\hat{c}(z))^{|D^-(z)|} \\
        = & \text{const} \cdot \log \prod_{z\in\Gamma} \left(\frac{\hat{c}(z)}{|D^+(z)|}\right)^{|D^+(z)|}\left(\frac{1-\hat{c}(z)}{|D^-(z)|}\right)^{|D^-(z)|}. \\
        \end{aligned}
      \end{equation}
      By the inequality of arithmetic and geometric means, we maximize the last line of Eq.\ref{eq:amgm} if and only if 
      $\frac{\hat{c}(z)}{|D^+(z)|}=\frac{1-\hat{c}(z)}{|D^-(z)|}$, hence $\hat{c}(z)=\frac{|D^+(z)|}{|D(z)|}$ minimize the cross entropy loss on training sample set $D$.
      Similarly, the optimal $c(z,\tilde{z})$ trained on $D$ is $c(z,\tilde{z})=\frac{|D^+(z,\tilde{z})|}{|D(z,\tilde{z})|}$. Therefore, the relation between the $\hat{c}$ of $\mathtt{M}_L$ and $c$ of $\mathtt{M}_H$ is
      
      \begin{equation}
        \begin{aligned}
        \hat{c}(z) = & \frac{\sum_{\tilde{z}}|D^+(z,\tilde{z})|}{|D(z)|} 
        = \sum_{\tilde{z}}\frac{|D^+(z,\tilde{z})|}{|D(z,\tilde{z})|} \cdot \frac{|D(z,\tilde{z})|}{|D(z)|} \\
        = & \sum_{\tilde{z}} c(z,\tilde{z}) \cdot \frac{|D(z,\tilde{z})|}{|D(z)|}.
        \end{aligned}
      \end{equation}
    \end{proof}
    
    % ----
    
    % 上述 prop 说明了在这个简单的场景中，同一个 ad user pair 预测出来的 dctr 和 pctr 之间具有某种关系
    The scenario in Proposition \ref{prop:two-ctr-relation} are simple, but we clarify that it is common seen in industrial online serving system. To guarantee the predictable performance and consistency of the whole system during online serving, different versions of prediction models for the same task are often trained on the same set of data samples, and have the same update schedule. 
    % 但是真实系统确实更加复杂，列举真实系统和上述的简单场景不同
    % (1) distillation 使得两个模型的 loss function 不同
    % (2) 真实的 feature space 实际不是连续的
    The main differences between the real system and the simple scenario in the Proposition \ref{prop:two-ctr-relation}. are (1) in the real system, the loss functions of the two models are different due to the usage of distillation techniques which aims at transferring the knowledge of the heavy model to the light model; (2) the feature space of the real world models is very large and complex, so we might not be able to derive a compact discrete representation like $\Gamma$ and $\tilde{\Gamma}$ in the simple scenario.
    % 虽然实际有点不同，但是我们可以从实际数据中观察到这样的结果
    Even the real system are more general from the simple scenario, we wildly observe the similar results in Eq.\ref{eq:dctr-vs-pctr} from the real system that, on the sample set with the same \emph{light feature} $z$, the average of the light model's output is often close to the average of the heavy model's output. 
    % 并且校准也会加强这样的结果的存在
    In fact, another assistant technique called calibration, which aims at aligning the average of the two models' outputs on the same \emph{light feature} $z$, also reinforces the relationship in Eq.\ref{eq:dctr-vs-pctr} between light model and heavy model. 
    
    % ----
    
    % Tentative 实现其实有不高效的地方
    \subsection{Inefficiency of TENTATIVE}
    
    We characterize the inefficiency of \emph{TENTATIVE} solution in this part. 
    % 首先，当 M=K 的时候，TENTATIVE 就是最优解
    First, we show the relationship between \emph{TENTATIVE} and the optimization problem \emph{SCP}. That is, when $M=K$, the \emph{TENTATIVE} is the optimal solution for \emph{SCP}.
    
    % 下面是 M=K 时，TENTATIVE 是最优解
    \begin{proposition}
    \label{prop:tentative-opt}
      When $M=K$, \emph{TENTATIVE} solution is optimal for problem \emph{SCP}. 
    \end{proposition}
    
    \begin{proof}
      When $M=K$, for a fixed $\sx_M\subseteq \sx_N$ that $|\sx_M|=M$  represented as $x=(x_1,...,x_N)\in 2^N$, the objective of the \emph{SCP} is 
      \begin{equation}
        \E_W[\mathtt{SumTopK}(\sx, W)] = \E_W[\sum_{j=1}^N x_j\cdot W_j] = \sum_{j=1}^N x_j \E_{W_j}[W_j].
      \end{equation}
      Therefore, the optimal subset $\sx_M^*$ selects the $M$ ad with the highest $\E_{W_j}[W_j]$. 
      From Proposition \ref{prop:two-ctr-relation}, $\hat{c}_j=\E[C_j]$. As $W_j=C_j\cdot v_j$ where $c_j\sim C_j$, then $\E_{W_j}[W_j]=\hat{c}_j\cdot v_j$. $\sx_M^*$ selects the $M$ as with highest $\hat{c}_j\cdot v_j$ which coincides the behavior of \emph{TENTATIVE}.
    \end{proof}
    
    % 但是当 M > K 的时候，TENTATIVE 就次优了，我们举个例子说明
    However, when $M>K$, \emph{TENTATIVE} is suboptimal. We illustrate the inefficiency of \emph{TENTATIVE} with a very simple example.
    \begin{example}
    \label{eg:tentative-subopt}
      There are $N$ ads ranked by their expected value $\E[W_1] \geq \ldots \geq \E[W_N]$. Ad $i\leq M$ has deterministic value $w_i$.  An ad $j>M$ has possible values $t\cdot \bar{w}_j$ and $\epsilon$ with probability $\frac{1}{t}$ and $1-\frac{1}{t}$ respectively, where $t$ is a large positive number that $t\cdot \bar{w}_j>w_K$ but $\E[W_j]=\frac{1}{t}\cdot t\cdot \bar{w}_j + (1-\frac{1}{t})\cdot \epsilon \leq \E[W_M]=w_M$.
      By the TENTATIVE solution, we select ad $1,\ldots M$ to form $\sx_M^{TEN}$ and obtain $\E_W[\mathtt{SumTopK}(\sx_M,W)]=\sum_{i=1}^K w_i$. However, if we select ad $1,\ldots M-1$ and $j$ to form $\sx_M'$, we obtain 
      $$\begin{aligned}
      & \E_W[\mathtt{SumTopK}(\sx_M',W)] \\
      = & \frac{1}{t}(\sum_{i=1}^{K-1} w_i + t\cdot \bar{w}_j) 
      + (1-\frac{1}{t})\cdot \sum_{i=1}^K w_i  \\
      > & \E_W[\mathtt{SumTopK}(\sx_M^{TEN},W)].
      \end{aligned}$$
    \end{example}
    
    % 这个例子看上去很奇怪，但是它实际上表达了
    % 我们实际上可以构造 K/M 的 worst case in general example  
    % 但是上面的例子是更加清楚地展示了 tentative solution 的实际状态：
    We can further construct an example that the tentative solution only achieves $\leq \frac{K}{M}$ fraction of the optimal objective, which is a worst-case performance of tentative solution in general case. However, the above example close to what really happens in this system: for a same sample, the predicted click through rate $c$ output by the heavy model $\mathtt{M}_H$ can be very different from the one output by the light model $\mathtt{M}_L$. With this observation, a intuitively better strategy for selecting $\sx_M$ when $M>K$ is to not only select average good ads but also some ads whose average value is not the top $M$ but with some probability at very high value which makes the ad to be top $K$.
    
    % TODO 这里需要从数据说明就是有很多方差极大的情况
    % TODO
    
    % ----
    
    % - 简单近似方法  
    % - 如果是把目标改为选中的个数，而不是 sw，那么是最优的  
    % - 这是一个多项式时间的算法  
    
    \section{A Simple Heuristic Solution}
    
    % TODO 总分
    % 首先证明 NP-hard，然后说想要 individual score function
    % 使用监督学习的技术：提出 2 个 loss，第 1 个很牵强的，第 2 个是随便弄的
    % TODO 还不能够用理论来证明他们之间的关系，只有靠实验了，尤其是 softmax cross entropy 不自洽
    % 然后介绍为了实现这个功能，使用的神经网络的结构
    
    \subsection{Complexity of pre-allocation decision}
    We first prove that the exact optimization of the \emph{SCP} is NP-hard.
    \begin{proposition}
    \label{prop:np-hard}
      The problem \emph{SCP} is NP-hard. 
    \end{proposition}
    \begin{proof}
      We prove that \emph{SCP} is NP-hard even when $K=1$ by reducing a well-known NP-hard problem set cover to \emph{SCP}.
      % 任意一个 set cover 实例
      We first define the general set cover problem. The world is $U=\{u_1, \ldots, u_A\}$ and there are a collection $T=\{S_1, \ldots, S_N\}$ where $\forall i\leq N$, $S_i\subset U$ is a subset of world $U$. The set cover problem is to decide whether there is a $T'\subset T, |T'|\leq M$ such that $\bigcup_{S_i\in T'}S_i=U$.
    
      % SCP 的一个实例
      Next, for any instance of the set cover problem, we define the corresponding \emph{SCP}. Given a set of random variables $W=\{W_1, \ldots, W_N\}$ where each $W_i$, corresponding to the above set $S_i$, has two possible values $\{0,1\}$. When all elements in $S_i$ are covered, $W_i=1$; otherwise, $W_i=0$.
      
      Therefore, there exists a $T'\subset T, |T'|\leq M$ if and only if there exists a $\sx_M$ with the expected maximum 1, i.e. 
      $$\E_W[\stk(\sx_M,W)]=1, \quad \text{for} \,\, K=1.$$
    \end{proof}
    
    % 可以看到问题的困难其实来自问题本身的组合性，还来自随机变量之间的复杂关系
    % 暴力的算法需要使用 N choose M 再乘上求期望时的 pctr^N 的集合的大小
    % 为了线上使用的可行性，我们想要一个能够对于每个 ad 进行单独评估的打分 f(x)，就像简单的 coarse pctr * bid 一样，而不是对于一个集合进行整体的打分
    % 注意个体打分函数也可以利用全局的信息，而不是单独的信息
    We see that the intractability of the \emph{SCP} mainly comes from that the intrinsic combinatorial structure of the problem and the dependence among the random variables. The direct brute force algorithm evaluates the set $\sx_M$, and the time complexity is $O\left({N \choose M}\cdot |\{pctr\}|^N \right)$, where $|\{pctr\}|$ is size of the set contains all possible $pctr$.
    
    \subsection{Learning based Score Function}
    For tractability and scalability in the online service usage, we wonder if we can design a individual score function, like the tentative solution score $\hat{c}_i \cdot v_i$, which evaluates each ad separably, instead of a set score function which evaluating the set $\sx_M$. 
    
    % 形式表述，大分函数 f【】将 pre-allocation 的全局信息 x 映射到所有N个广告的自己的得分
    % 即 f 将 x 映射一个排列
    % 为了使得 f 能够优化 SCP，f 的前 M 需要尽可能覆盖正式拍卖中的 pctr * bid 的前 K 名
    % 但是这个排列空间的指数大小使得直接设计 f 变得很困难
    % 于是我们利用神经网络近似复杂映射和分布的能力，通过学习来设计参数化的 f
    % 记训练数据集为 D_f，预分配模块的输入 x 作为训练特征，正式拍卖中的 ecpm 作为训练标签
    % 我们采用监督学习的方法，最小化经验损失函数 L，其中 l 是局部损失函数
    % 下面我们介绍两种有效的局部损失函数：（1）交叉熵损失，（2）优化 top K 命中率的损失函数
    
    Formally, this individual scoring function $f:\mathcal{X}^N \rightarrow \mathbb{R}^N$ maps the global information $x$ of the pre-allocation decision module to $N$ individual scores, where $f_i(x)$ is the score for ad $i$. 
    As we rank in pre-allocation decision by $f_i$s and select the top $M$ ads as $\sx_M$, $f$ actually maps $x$ to a permutation. 
    To let the permutation induced by $f$ serve SCP optimization, the top $M$ $f_i$s should cover as much ads with largest $K$ formal auction scores $pctr\cdot bid$ as possible. 
    The exponential size of permutation space makes a direct design of individual score function $f$ intractable.
    Therefore, we leverage neural networks' strong ability on encoding complex mapping and distribution, to learn parametrized individual function $f(\cdot;\theta)$.
    Denote the training data set as $D_f=\{(x,y)\in \mathcal{X}^N\times \mathbb{R}^N\}$, where the feature $x$ is the input to pre-allocation decision module, and the label $y$ is the $pctr\cdot bid$ in formal auction stage.
    We adopt supervised learning to train scoring function $f$ by minimizing the empirical loss 
    $$L(f)=\frac{1}{|D_f|}\sum_{(x,y)\in D_f} l(y,f(x)),$$
    where $l(y,f(x))$ is the local loss function for each sample.
    Next, we propose two effective local loss functions for training the parametric individual score function $f(\cdot;\theta)$: 
    (1) softmax cross-entropy loss; 
    % (2) lower bound surrogate loss for social welfare; 
    (2) exact loss for top $K$ accuracy. 
    
    \subsubsection{Softmax cross-entropy loss}
    % top one 交叉熵 loss
    % 实际上，给定集合所有元素的特征，建立到排列空间的映射，是 ltr 领域研究的内容
    % softmax cross-entropy 是它里面一个在实践中广泛有效的近似方法
    % 它是
    % 这个loss可以解释为基于 y 和 fx 给出的 top one 分布之间的交叉熵
    % 这个损失函数来自于 learning to rank
    In fact, the problem of mapping features from all set elements into the space of permutations with supervised learning is studied under a machine learning area called \emph{learning to rank} \cite{liu2011learning}.
    This softmax cross-entropy loss is a common practical and effective loss from this area \cite{cao2007learning, xia2008listwise}.
    \begin{equation}
    \label{eq:listnet-loss}
      l(y,f(x)) = -\sum_{i=1}^N \frac{\exp(y_i)}{\sum_{j=1}^N \exp(y_j)} \log \frac{\exp(f_i(x))}{\sum_{j=1}^N \exp(f_j(x))}.
    \end{equation}
    Eq.\ref{eq:listnet-loss} can be interpreted as the cross entropy between two probability distributions,
    $$ P_{y,i} = \frac{\exp(y_i)}{\sum_{j=1}^N \exp(y_j)}, P_{f(x),i} = \frac{\exp(f_i(x))}{\sum_{j=1}^N \exp(f_j(x))},
    $$
    where $P_{y,i}$ and $P_{f(x),i}$ represents the probability of ranking ad $x_i$ to the top of $x$ given the $N$ scores $y$ and $f(x)$ respectively.
    
    % \subsubsection{Lower bound surrogate loss for social welfare}
    % % 这个损失函数是通过分析 scp 问题本身，然后构造的一个 social welfare 优化的下届指标
    % % 固定一个 M 集合，scp 的目标函数【】
    % % 记号表示【】
    % % 第三个等号是因为固定了 W 的取值之后，如果一个广告牌在集合 M 之中，同时又在 N 集合的前 K 那么这个它一定在 MK 中。
    % We derive this local loss function by first analyzing the \emph{SCP} problem itself and then constructing a surrogate score metric which lead to a lower bound of the original \emph{SCP}. 
    % Fix a selected set $\sx_M$, then the objective value of \emph{SCP} is
    % \begin{equation}
    % \label{eq:sw-score-hard}
    % \begin{aligned}
    %   & \E_{W|x}[\mathtt{SumTopK}(\sx_M,W)] 
    % =  \sum_{i\in \sx_N} \E_W[\mathbf{1}[i\in \sx_M^K] \cdot W_i] \\
    % = & \sum_{i\in \sx_N} \E_{W|X}[ 
    %   \mathbf{1}[i\in \sx_M^K \cap \sx_N^K]\cdot W_i + 
    %    \mathbf{1}[i\in \sx_M^K \backslash \sx_N^K]\cdot W_i] \\
    % = & \sum_{i\in \sx_M} \E_{W|X}[\mathbf{1}[i\in \sx_N^K]\cdot W_i] + 
    %     \sum_{i\in \sx_M} \E_{W|X}[\mathbf{1}[i\in \sx_M^K \backslash \sx_N^K] \cdot W_i],
    % \end{aligned}
    % \end{equation}
    % where $\sx^K$ means the top $K$ values of $W_i$ in set $\sx$. The first equality is due to the linearity of expectation. 
    % For the third equality, fix any realization of $W$, if the ad $i$ is the top $K$ in the $\sx_N$ then the ad $i$ is must in the top $K$ of $\sx_M$ as $\sx_M\subset\sx_N$, i.e. $\forall i\in \sx_M$, $\mathbf{1}[i\in \sx_M^K \cap \sx_N^K]=\mathbf{1}[i\in\sx_N^K]$. 
    
    % % 这个东西再次告诉我们为什么在 M > K 的时候难以得到一个 separable score
    % % 但是我们可以由上面的第一项构造一个原始优化目标的下届 【】
    % % 他只考虑是 NK 的广告对于 MK 的前 K 作出的贡献
    % % 根据这个下届目标，我们可以得到个人的大粉函数，他计算个体广告进入 N 集合的 K 时的期望价值，在 W|x 分布上求期望
    % Eq.\ref{eq:sw-score-hard} illustrates that hardness of design a evaluation score for each ad separably is intuitively due to that we cannot remove the $\sx_M^K$ in the expectation operation from the second term in the last line when $M>K$.
    % However, from the first term in the last line of Eq.\ref{eq:sw-score-hard}, we can construct a lower bound of the original \emph{SCP} objective as
    % $$\E_{W|x} [\stk(\sx_M,W)] \geq 
    % \sum_{i\in\sx_M}\E_{W|x}[\mathbf{1}[i\in \sx_N^K]\cdot W_i],$$
    % which considers only the social welfare contributed by the top $K$ ad $i\in\sx_N^K$ who enters $i\in\sx_M$, \ie, $i\in\sx_M^K\cap\sx_N^K$.
    % From this surrogate lower bound objective, we obtain an individual evaluation score which measures the expectation of ad $i$'s valuation when enters set $\sx_N^K$ over conditional distribution of all ads' valuations given their feature $x$,
    % \begin{equation}
    % \label{eq:heuristic-sw-score}
    %   f_i(x) = \E_{W|x}[\mathbf{1}[i\in \sx_N^K]\cdot W_i].
    % \end{equation}
    % Then we can select $\sx_M$ by first computing $f_i$ for all $i\in\sx_N$ and then selecting the ads corresponding to the $M$ highest $f_i$'s.
    
    % % 由于计算 f_i 需要 Pr[W|x] 的分布，我们下面建立概率模型，从而可以使用极大似让的方法直接参数化近似出 f
    % % 
    % % As directly computing $f_i(x)$ requires distribution $Pr[W|x]$, we build probabilistic model, so that we can encoding both the function $f$ and its dependent distribution of $Pr[W|x]$ into a parametrized neural networks by maximizing likelihood estimation.
    % % Define random variable vetor $B=(B_1,\ldots, B_N)$, where $B_i=\mathbf{1}[i\in\sx_N^K(W)]\cdot W_i$ is based on random variable vector $W$.
    % % 写不下去了，丢掉
    
    \subsubsection{Exact loss for top $K$ accuracy}
    % 我们考虑另一个优化问题，即优化 pre-allocation 中的前 K 的命中率
    % 注意这个问题和优化 social welfare 是很接近的
    % 但是我们可以直接通过问题本身推导出一个 individual score function 
    % 考虑固定一个选定的集合 M，那么他的期望 top K 命中率是
    % 其中记号表示，等式表示
    We turn to another problem of optimizing top-$K$ accuracy in pre-allocation decision module, \ie, to make $\sx_M$ cover as much ads in $\sx_N^K$ as possible in expectation,
    $$\max_{\sx_M(x)} \quad \E_{W|x}[\stk(\sx_M(x), \{\mathbf{1}[i\in\sx_N^K]\}_{i\in\sx_N})].
    $$
    Note that this problem is closely related to optimizing social welfare, but we can naturally derive a individual metric $f_i^a$ for selection $\sx_M$ by ranking with the $f_i^a$ and truncating at rank $M$ under top-K accuracy optimization.
    Consider fixing a selected set $\sx_M$, then the expected top-$K$ accuracy is
    \begin{equation}
    \label{eq:acc-score-easy}
    \begin{aligned}
      & \E_{W|x}[\stk(\sx_M,\{\mathbf{1}[i\in\sx_N^K(W)]\}_{i\in\sx_N})] \\
      = & \sum_{i\in \sx_N} \E_{W|x}[\mathbf{1}[i\in \sx_M^K(W)\cap\sx_N^K(W)]] \\
      = & \sum_{i\in \sx_M} \E_{W|x}[\mathbf{1}[i\in \sx_N^K(W)]] \\
      = & \sum_{i\in \sx_M} \Pr_{W|x}[i\in \sx_N^K(W)],
    \end{aligned}
    \end{equation}
    where $\sx^K$ means the top $K$ values of $W_i$ in set $\sx$. The first equality is due to the linearity of expectation; the second equality is due to that fix any realization of $W$, if the ad $i$ is the top $K$ in the $\sx_N$ then the ad $i$ is must in the top $K$ of $\sx_M$ as $\sx_M\subset\sx_N$, i.e. $\forall i\in \sx_M$, $\mathbf{1}[i\in \sx_M^K \cap \sx_N^K]=\mathbf{1}[i\in\sx_N^K]$. 
    
    % 于是得到一个优化 topk 准确率的个体大粉函数
    % 于是我们可以通过排序这个分来选择最高的 M 组成 M 集合
    Hence, we have a individual score function $f_i^a$, which maximizes the expected top-K accuracy, as
    \begin{equation}
    \label{eq:exact-acc-score}
      f_i^a(x) = \Pr_{W|x}[i\in\sx_N^K(W)].
    \end{equation}
    Then, we can select $\sx_M$ which exactly maximizes the expected accuracy of top-$K$ accuracy by first computing $f_i^a$ for all $i\in\sx_N$ and then selecting the ads corresponding to the $M$ highest $f_i^a$ values.
    
    % 由于计算 f_i^a 需要 Pr[W|x] 的分布，这个分布可能有复杂的依赖关系
    % 为了避免这个，我们下面建立概率模型，从而可以使用极大似让的方法直接参数化近似出 f
    However, direct computation of $f_i^a(x)$ requires explicit distribution $\Pr[W|x]$, which might be complex with unknown interdependent structure. 
    To avoid this, we build probabilistic model, so that we can encoding both the computation logic of function $f^a(x)$ and the required distribution of $\Pr[W|x]$ into a parametrized neural networks $f^a(x;\theta^a):X^N \rightarrow [0,1]^N$ by maximizing likelihood estimation.
    % 定义随机变量 $B$
    % 假设给定了全局的 x 和额外的信息 tilde x 之后，B_i 之间是相互独立的，是伯努利的分布，具有一个参数
    % 我们使用 f^a(x theta^a) ，利用极大似然估计这个二分类的变量
    % 得到一个 N 求和的 二分类交叉熵
    Define a random variable vector $B=(B_1,\ldots,B_N)$ that $B_i=\mathbf{1}[i\in \sx_N^K(W)]$. 
    We assume that after giving the global $x$ and another auxiliary information $\tilde{x}$ as the condition, random variables $B_i$ in $B$ are independent, \ie, $\Pr[B=b|x,\tilde{x}]=\prod_i \Pr[B_i=b_i|x,\tilde{x}]$, which means $B_i|x,\tilde{x}$ is a univariate Bernoulli distribution with parameter $\Pr[B_i=1|x,\tilde{x}]$
    Next we use $f_i^a(x)$ to approximate the Bernoulli parameter of $\Pr[B_i=1|x,\tilde{x}]$, then we maximize the log likelihood on the data set,
    \begin{equation}
    \label{eq:b-bernoulli}
      \begin{aligned}
      & \sum_{j\in D_f} \log \Pr[x^{j},b^{j}|f^a(x,\theta)] \\
      = & \sum_j \log \prod_i \Pr[x^{j},b^{j}_i|f^a(x,\theta)] 
      = \sum_{i,j} \log \Pr[x^{j},b^{j}_i|f^a(x,\theta)] \\
      = & \sum_{i,j} ( b^{j}_i \log \Pr[b^{j}_i=1|x^{j}] 
       + (1-b^{j}_i) \log (1-\Pr[b^{j}_i=1|x^{j}]) ) \\
      = & \sum_{i,j} ( b_i^{j} \cdot \log f_i^a(x^j;\theta^a) 
        + (1-b^{j}_i) \cdot \log (1-f_i^a(x^j;\theta^a)) ),
      \end{aligned}
    \end{equation}
    where $b^j_i$ means $\mathbf{1}[i\in\sx_N^K(w^j)]$ corresponding to sample $(x^j,w^j)$ from data set $D_f$.
    If we negate Eq.\ref{eq:b-bernoulli}, then we obtain a local function as Eq.\ref{eq:acc-loss} with a form of summation on $N$ binary classification cross entropy loss, which guides $f_i^a(x;\theta^a)$ to approximate $\Pr_{W|x}[i\in\sx_N^K(W)]$.
    \begin{equation}
    \label{eq:acc-loss}
      l(y,f(x)) = -\sum_{i=1}^N ( b_i\log f_i^a(x;\theta^a) + (1-b_i)\log (1-f_i^a(x;\theta^a)) ).
    \end{equation}
    
    \subsection{Networks with Set Encoding}
    
    In our probabilistic modeling for $f(x)$ and $f^a(x)$, the feature $x$ from the whole set of ads are used to determine each ad $i$'s individual score. We adopt the network architecture introduced by Deep Sets \cite{zaheer2017deep} which aggregates individual ad features in a permutation-invariant manner.
    \begin{figure}[h]
      \centering
      \includegraphics[width=\linewidth]{./21fupa_main_wsdm/fig/networks.pdf}
      \caption{Network architecture of PAD. The encoding net receives every ad's raw feature and outputs its individual encoding. Then we aggregate individual encodings into a global encoding, and send the concatenation of raw ad feature and the global encoding to the score net.}
      \Description{}
      \label{fig:networks}
    \end{figure}
    As shown in Fig.\ref{fig:networks}, every ad is first encoded in a \emph{encoding net} as an individual encoding. Then the $N$ individual encodings are aggregated in a global encoding with permutation invariant operators such as \texttt{mean}, \texttt{min}, \texttt{max} . Then, we concatenate the aggregated global encoding to the raw feature of each individual ad and use a light dense network to \emph{score net} for each ad in the global set.
    Note that, both the \emph{encoding net} can work with $N$ ads in parallel, and after the global encoding aggregation, the \emph{score net} can also work in parallel for $N$ ads. 
    Therefore, the PAD networks can achieve a high throughput.
    Specifically, we call the PAD network trained with softmax cross entropy loss as PAD-sw and the other trained with the exact loss for top $K$ accuracy as PAD-acc.
    Note that due to the existence of global encoding, the PAD-sw networks is different from traditional learning to rank where the canonical rank score only depend on the individual item itself.
    For the PAD-acc networks, the global encoding is also very important because in our probabilistic modeling, we assume that $B_i=\mathbf{1}[i\in\sx_N^K]$s are independent when the global set information $x$ is given. Here, the global encoding works as a compact representation of $x$.
    
    \section{Empirical Evaluation}
    
    % 基本设置
    % 数据
    % 评价指标
    % 对比方法：解释
    % 模拟设置
    
    \subsection{Evaluation Setting}
    
    \subsubsection{Data setting}
    % 我们随机选择了时间和数据
    % 数据来自于一次 empirical observation 设置了
    % 由于这是拍卖系统正式拍卖阶段搜集的数据，所以具有这些特征
    % 注意这些数据是拍卖系统决策模块的数据，比预测模块的数据少多了
    The dataset we used for evaluation comes from \emph{Taobao}, a leading e-commerce advertising system in China. We randomly sampled 24K auction records logged data from January 8th 12-14pm 2021 as training data, and 6K auction records logged data from the same time period as testing data. 
    All the data are collected from the two-stage auction system during an online environment of setting the size of the candidate ad set to the formal auction stage as 700.
    Therefore, for each of this 700 ads, we have the below features:
    (1) prediction results from the light and coarse prediction module in the pre-allocation stage, such as $\hat{pctr}$, $pcvr$ (predicted conversion rate) and some historical statistics such as historical click through rate and conversion rate; (2) prediction results from the heavy and fine prediction module, such as $pctr$; (3) ad information like $bid$, category of the product, price of the ad product, type of marketing aim of the advertiser.
    Recall that the prediction modules in both the pre-allocation stage and the formal auction stage depend on highly aggregated information from the corresponding prediction modules, instead of directly requiring the large amount of raw user and ad features, therefore, both the decision modules are much lighter than even the light prediction module.
    
    \subsubsection{Evaluation metrics}
    
    We consider the following metrics in our experiments.
    \begin{itemize}
      \item Social welfare rate: $swr=\frac{\sum_{i\in \sx_M^K}pctr_i \cdot bid_i}{\sum_{j\in \sx_N^K} pctr_j \cdot bid_j}$.
      \item Top K Accuracy: $acc={\sum_{i\in \sx_M^K}\mathbf{1}[i\in \sx_M^K\cap \sx_N^K]}$.
      \item CTR rate: $pctrr=\sum_{i=1\in\sx_M^K} pctr_{(i)}/\sum_{i=1\in\sx_N^K} pctr_{(i)}$.
      \item Revenue rate: $revr={rev(\sx_M^K)}/{\sx_N^K}$, where revenue $rev$ is under GSP auction and the subscript $(i)$ means the bidder with the $i$-th highest value of $pctr \cdot bid$.
      $$rev(\sx^K)=\sum_{i=1}^K pctr_{(i+1)} \cdot bid_{(i+1)}.$$
      
    \end{itemize}
    Ad revenue is an important metric when we evaluate an auction system. 
    As our main optimizing target, social welfare, is an upper bound of revenue, we also concern the influence on revenue when we improving the social welfare.
    As auction system is a multi agent system with strategic bidders, revenue is often considered under a stationary state of the system, such as under the Nash equilibrium.
    Recall that we assume the bidders in this online advertising system are value maximizers \cite{wilkens2017gsp}, \ie a bidder aims at maximizing the value of the ad positions she wins, instead of maximizing her value minus her payments. Under this rational assumption model of bidders, GSP auction is incentive compatible, \ie, every bidder is willing to report their truthful values.
    Therefore, we can regard the bid logged in this system which runs GSP mechanism is stable as it truthfully reflects the bidder's stable truthful value for a user click in recent period.
    
    \subsubsection{Methods for Comparison}
    
    We introduce methods for comparison as below. 
    As all the methods are in a \emph{scoring and truncating} fashion, we mainly describe their rank score function.
    \begin{itemize}
      \item TENTATIVE solution (TEN): As we described in previous section, the rank score is $\hat{pcrt}\cdot bid$ where $\hat{pctr}$ is output by the light prediction module in the pre-allocation stage.
      
      \item Point-wise $pctr$ regression (REG-P): We use ground truth fine $y=pctr$ as label, and use the input feature to the each individual ad in pre-allocation decision module to train a light weighted regression model with mean square loss. The word point-wise means we provide no global information to the model. The rank score function for selecting subset is $\tilde{pctr}^P\cdot bid$, where $\tilde{pctr}^P$ is output by the regressor.
      
      \item $pctr$ regression with global set information (REG-S): The differences between REG-S and REG-L is that REG-S has additional global set information as model input to train the regression which output $\tilde{pctr}^S$. REG-S adopts a neural networks architecture as Fig.\ref{fig:networks}. The rank score function is $\tilde{pctr}^S\cdot bid$. 
    \end{itemize}
    
    \subsubsection{Simulation setting}
    % 看了撬动的写法
    % 我们使用真实数据搭建了模拟环境
    % 由于真实数据存下来了bid和两个阶段中的预估值对于所有的广告，所以我们可以通过重新回放数据的方法来评估方法  
    % 这种离线评估的方法在研究工作中非常常见
    % 由于我们的目标是评估 pre allocation 中的决策方法，我们将正式拍卖阶段固定为和收集线上数据时线上环境一样的 GSP 拍卖  
    We conduct empirical evaluation in simulation environment based on the real industrial data setting described as above. As we have stored for every ad in the initial candidate set $\sx_N$ the $bid$ as well as the prediction results $\hat{pctr},pctr$ from prediction modules in both the pre-allocation stage and the formal auction stage, we are able to train and test our methods by replaying the data in an offline fashion. 
    As our purpose is to evaluate the pre-allocation decision module, we fix the formal auction stage as the same as the online setting where we collected our base data sets, \ie running GSP auction based on $pctr\cdot bid$ to determine the allocation and payment of the ad positions.
    
    \subsection{Performance Comparison}
    % 我们对比 PAD 和其他方法的性能指标
    % 见 table perf
    % 我们提出的 pad 系列的方法都超过了 tentative 的方法
    
    Table.\ref{tab:perf} shows the performances of our proposed PAD methods with the baseline methods.
    
    First, we can see that our PAD-sw and PAD-acc achieves the best performances on all evaluation metrics. This result verifies the motivation that improvement in matching efficiency, \ie expected clicked social welfare in pre-allocation stage, benefits the three roles in the advertising system, \ie the users, the advertisers and the ad platform.
    
    Second, we can see that both of our proposed PAD methods outperform the tentative solution in both the social welfare and accuracy in top $K$ by a clear margin. This verifies our motivation of using PAD to implicitly model the relationship between the feature of the pre-allocation decision module with the $pctr$ from the heavy prediction module $\M_H$ in the later formal auction stage.
    
    Third, we provide empirical evidence suggesting the meaningfulness of set encoding. 
    In the last two lines of Table.\ref{tab:perf}, we conduct experiment after disabling the set encoding module in PAD networks, named PAD-acc(w/o set) and PAD-sw(w/o set). 
    This phenomenon indicates that PAD networks can leverage the correlation among the $N$ ads in the same request to improve its implicit modeling of the distribution of $pctr$ in later formal auction and also use the global information in the initial candidate set to help PAD distinguish potential proper ads in the context of the total initial candidate set.
    
    \begin{table}[!t]
      \caption{The comparison results of different methods in simulation experiments. $N=700, M=30, K=5$.}
      %\vspace{-0.6em}
      \small
      \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    % \multirow{2}*{} & \multicolumn{2}{c|}{with set encoding} 
    %               & \multicolumn{2}{c|}{w/o set encoding} \\ \cline{2-5} 
               & $swr$ & $acc@K=5$ & $pctrr$ & $revr$ 
    \\ \hline
    TEN  & 0.7819 & 1.8786 & 0.6834 & 0.9099 
    \\ \hline
    REG-P & 0.8011 & 1.9376 & 0.6928 & 0.9359
    \\ \hline
    REG-S & 0.8238 & 2.1068 & 0.6966 & 0.9659
    \\ \hline
    PAD-acc    & 0.8414 & 2.2869 & 0.7274 & 0.9847
    \\ \hline
    PAD-sw     & \textbf{0.8461} & \textbf{2.3262} & \textbf{0.7412} & \textbf{0.9932}        
    \\ \hline
    PAD-acc(w/o set)    & 0.7899 & 1.8142 & 0.6371 & 0.9152
    \\ \hline
    PAD-sw(w/o set)     & 0.8251 & 2.1072 & 0.6882 & 0.9647
    \\ \hline
    
    \end{tabular}
    \label{tab:perf}
      %\vspace{-0.6em}
    \end{table}
    
    \subsection{Incentive Property of PAD}
    % 由于 PAD 服务的决策环境是拍卖系统中，一部分
    As PAD works in an advertising auction system where there are rational bidders who might misreport their valuation to a user click for their own benefits, the whole auction system should ensure the property of incentive compatibility which encourages the bidders to truthfully report their valuation to a user click as their bid. 
    We mentioned before that the rational bidder model assumption in this system is value maximizer bidder. A conclusion in auction theory about this type of value maximizer bidder is that any auction mechanism with allocation monotonely non decreasing according to bid is incentive compatible to bidders.
    As we use GSP auction in formal auction stage, which satisfies this monotonicity, to analyze the incentive property of the whole system, we need to analyze whether the pre-allocation stage is also monotonely non decreasing.
    
    We conduct counter factual perturbation on bidder's bid in the log, which is also used in incentive property testing \cite{deng2019testing,deng2020data}, and then simulate the two-stage with the perturbation to check the monotonicity of the PAD.
    Specifically, in each counter factual test, we sample one auction from the test data set, and sample one ad $j$ in this auction. Then, we apply a set of multiplication factor $\alpha\in \{0.1 \times i|i=1,\ldots,20\}.$ and replace $bid_j$ of the sampled ad $j$ to $\alpha\cdot bid_j$. Next, we simulate the auction again to see if there are violation of (a)\emph{monotonely non-decreasing allocation according to bid}, and a also strong requirement as (b)\emph{monotonely non-drop rank according to bid}.
    For either of PAD-rank and PAD-acc, we sample 1000 auctions from testing data and 10 ads from each auction. 
    The low ratio of violation in Table.\ref{tab:ic-violation} means that even we add no deliberate design on PAD for a guarantee of strictly non-decreasing allocation according to bid, the learning based PAD methods satisfy it to some extend automatically. Intuitively, this is due to that supervised data include a signal that bid has a positive effect on the rank.
    
    \begin{table}[!t]
      \caption{Violation ratio in perturbation test. }
      %\vspace{-0.6em}
      \small
      \centering
    \begin{tabular}{|c|c|c|}
    \hline
             & PAD-acc & PAD-sw  
    \\ \hline
    type (a)  & 0.0 & 0.0  
    \\ \hline
    type (b) & 0.0 & 0.0031
    \\ \hline
    
    \end{tabular}
    \label{tab:ic-violation}
    \end{table}
    
    
    \section{Conclusion}
    In this work, we study the problem of pre-allocation decision in a two-stage online advertising auction system, where the ability gap between the different prediction modules in two stages causes inefficient user-ad matching and loss of social welfare. 
    We target to design a pre-allocation decision solution for social welfare optimization in two-stage auction system.
    In the first step, we give a formal definition to this problem as a stochastic combinatorial programming.
    Then, we illustrate the inefficiency of a canonical implementation in practice by analyzing the relationship between the two prediction modules.
    Next, as we can reduce the problem to NP-hard set cover, we proposed learning based PAD networks which leads to a practical approximate solution.
    In our empirical evaluation on industrial data set, PAD demonstrates highly positive effect on social welfare, and also on metrics according user experience and ad platform revenue.

==> 21fupa_main_wsdm/fig/21fupa_conclusion.tex <==
\section{Conclusion}

% 这个工作研究了新颖的问题：设计两阶段的电商广告拍卖系统，这里包括拍卖机制和用户行为预测模型。  
% 我们形式化设计两阶段拍卖，包括 预拍卖和拍卖，优化社会福利的问题。  
% 展示了一种常见设计中，因为 pre-auction 问题定义不合适，忽略了预拍卖和拍卖两阶段之间的关系，从而造成的社会福利损失。  
% 由于我们提出的预拍卖形式化是一个 NP-hard 的带限制次模优化，我们使用基于学习的方法求出近似解，叫做 PAS。  
% 在公开数据和工业数据上的实验证明了 PAS ，相比不恰当的问题定义而言，能够提升 two-stage auction system 的

In this work, we study a novel problem of designing two-stage auction system, which consists with auction mechanism and user behavior estimator, for large scale e-commerce advertising. 
We formulate the problem of designing two-stage auction mechanism, including pre-auction stage and auction stage, for social welfare maximization. 
We illustrate social welfare loss of a canonical tentative implementation due to improper formulation of pre-auction stage, as it ignores the relationship between the pre-auction stage and auction stage.  
As the our proposed formulation of pre-auction stage is an NP-hard problem of submodular maximization with cardinality constraints, we propose a learning based approach, called Pre-Auction Score (PAS) as a practical approximate solution.  
Experiment results on both public and industrial dataset demonstrate significant positive effect of PAS on social welfare, and revenue of the two-stage auction system, than the canonical solution which ignores the relationship between the two stages.   

% ====

==> 21fupa_main_wsdm/fig/21fupa_exp.tex <==
\section{Experiments}

In this section, we provide empirical evidence to demonstrate the insight in Section. 4. and the effectiveness of our proposed two-stage auction system. 
We conduct experiments on both public dataset and industrial dataset. 

\subsection{Settings for Public Dataset}

% 公开数据集上面的设定  
% 【从 DIN 抄的过来的】  
% Amazon 数据集包括亚马逊的商品评论和元数据。  
% 我们在实验中使用子集 Books，包含【】数量的用户商品类目和【】样本。  
% 我们把用户评论当作用户行为，把物品当作广告。  
% 用户特征包含用户 id，用户历史浏览列表，每个元素包含物品和类目的 id。
% 每个用户的长度是 >= 5 的。  
% 物品特征包含【】。  
% 我们基于 Amazon 数据集中的 用户-广告 交互数据模拟两阶段拍卖，模拟两阶段拍卖，生成了 40000 场拍卖。
% 每场拍卖中有 1000 个随机选择的广告。  
% 每个广告的出价是均匀分布独立采样。
% 我们定义用户的部分特征是用户 id 和评论序列的前三个商品【】。
% 部分的广告的特征和完全的物品特征是一致的。

The public dataset Amazon Dataset \footnote{http://jmcauley.ucsd.edu/data/amazon/} contains product reviews and metadata from Amazon \cite{he2016ups,mcauley2015image}. 
We conduct experiments on the subset called Books, which contains 603,668 users, 367,982 items, 1,600 categories and 603,668 reviews.
We regard reviews as user clicks and regard items as ads.  
The full features of a user $u$ include user\_id, and a list of user's reviewed items along with categories in history, \ie hist\_items\_id, and hist\_cate\_id. 
Each user's list contains at least 5 reviews. 
The full ad features $a_i$ consists of the item\_id and its cate\_id. 
Based on these user-ad interaction from the dataset, we simulate the process of two-stage auction and generate 40,000 auctions record data. 
In each auction, there are 1,000 randomly selected ads. 
The bid of each ad is sampled from uniform distribution independently. 
We define the partial user feature $\tilde{u}$ as user\_id and the first three item in the user's history review list, \ie hist\_items\_id[:3], hist\_cate\_id[:3].
The partial ad features $\tilde{a}_i$ is defined the same as the full ad features $a_i$. 

% 为了模拟第二阶段的正式拍卖，我们使用用户和广告的完全特征训练 深度兴趣网络 DIN ，一个电商平台点击率预估的预估器，作为精细的预估器输出 ctr，然后我们可以为每个广告生成标签 bid * ctr。 
% 为了构建用于对比的 ten 方法，我们使用用户和广告的部分特征来训练 FCN，输出 tilde ctr。
%【TODO 是否需要画图，因为要开源代码，就不详细写 DIN 和 FCN】。  
% 训练 DIN 和 FCN 的数据完全相同，即相同的用户广告对和相同的随机生成 1:1 的正负样本。
% 设降采样率为 eta，则 ctr 由神经网络的输出经过公式【】得到。
% 对于 ctr 和 tilde ctr 都要分别使用 DIN 和 FCN 的输出使用公式【】得到。
% 我们考虑两个降采样率分别为 0.01 和 0.05，记为设定 Public-1 和 Public-5。

To simulate the second stage of auction, we use full user and ad features $(u,a_i)$ to train Deep Interested Networks (DIN), a baseline $ctr$ estimator in e-commerce platform \cite{zhou2018deep}, as the refined and heavy model $\M^r$ to generate $ctr(a_i,u)$ for each ad, then we can generate label $b_i\cdot ctr(a_i,u)$ for each ad. 
To simulate the Tentative method for comparison, we use user and ad's partial features $(\tilde{u},\tilde{a}_i)$ to train a Embedding + Max Pooling + Fully Connected Network model (FCN), as the coarse and light model $\M^c$ to generate $\tilde{ctr}(\tilde{a}_i,\tilde{u})$ for each ad.  
The training samples for $\M^r$ DIN and $\M^c$ FCN are the same, \ie the same pairs of user and item from review dataset as positive sample, along with the same 1:1 negative samples. 
Let the negative down sampling rate be $\eta$.
When the estimator network trained with 1:1 negative samples output $p$, then the calibrated $ctr$ is 
$ctr=\frac{p}{p+(1-p)/\eta}$ \cite{he2014practical}. 
We consider two negative down sampling rate, $0.01$ and $0.05$, and denote the two settings as Public-1 and Public-5, respectively.
\input{./21fupa_main_wsdm/21fupa_fig_br.tex}

\subsection{Settings for Industrial Dataset}

% 我们随机选择了时间和数据
% 数据来自于一次 empirical observation 设置了
% 由于这是拍卖系统正式拍卖阶段搜集的数据，所以具有这些特征

% 工业数据来自一个领先的电商平台的两阶段的广告拍卖系统的运行记录。
% 我们随机选择了 2021年1月8日 12pm-14pm 的 30,000 场拍卖纪录。
% 每个拍卖纪录中，有 700 个广告，每个广告的特征包括：
% （1）粗糙预估器的 tilde ctr 和一些历史统计的平均 ctr 和 cvr。我们吧这些预估的信息看作是用户和广告的信息的聚合；（2）广告信息比如说 bid 和类目商品的售价和召回类型。
% 精细预估器输出的 ctr 用于生成标签 bid * ctr。

The industrial dataset we use for experiment comes from the log of a two-stage ad auction system in a leading e-commerce platform.
This two-stage ad auction system runs with TEN method, \ie a coarse but light ctr estimator $\M^c$ works in the pre-auction stage using partial user and ad features, while a refined but heavy ctr estimator $\M^r$ works in the auction stage using full user and ad features. 
We randomly sample 30K auction records logged data on January 8th 12pm to 14pm 2021. 
In each auction, there are 700 ads. 
For each ad, the features are: 
(1) $\widetilde{ctr}(\tilde{a}_i,\tilde{u})$ from $\M^c$, some historical statistics such as historical averaged refined $ctr$ and $cvr$ of this ad. 
We regard this estimated value as the cross features of the partial user and ad features $(\tilde{a}_i,\tilde{u})$; 
(2) Ad information like bid $b_i$, category and selling price of the goods associated with the ad, and the reason for match the ad to the user as a candidate for this ad auction (match\_type). 
The estimated $ctr(a_i,u)$ from $\M^r$ are used to generate label $b_i\cdot ctr(a_i,u)$.

\begin{comment}
% 注意这些数据数据只包含高度整合过的预估值，而不包含原始特征。  
% 我们可以把这个工业数据中的设定下的实验，看作包含了公开数据集 pre-auction 基于原始特征的设定的一个互补。  
% 由于特征都很少，所以可以使用一个非常轻量级的神经网络来近似打分函数。  
% 【TODO 神经网络的具体配置】  

Note that this industrial dataset only explicitly records highly aggregated information of the user such as estimated $\widetilde{ctr}$, $ctr$ and $cvr$, instead of the user id and the shopping history. 
We can regard setting on this industrial dataset as a complementary to the setting in the public dataset with raw user and ad features. 
As the features are several scalars (\eg $\widetilde{ctr}$, $cvr$) along with several low dimensional categorical features (\eg match\_type, cate\_id), we can use very light-weighted individual score networks, which depends on the existing light-weighted coarse $\M^c$ and $cvr$ estimator. 
\end{comment}

\input{./21fupa_main_wsdm/21fupa_tab_perf_pub_01.tex}
\input{./21fupa_main_wsdm/21fupa_tab_perf_pub_05.tex}
\input{./21fupa_main_wsdm/21fupa_tab_perf_ind.tex}

\subsection{Methods for Comparison}

% 为了证明我们的 pre-auction 设计的有效性，我们介绍下面的方法用于比较。
% 由于所有方法都是先排序后切断的方法从 N ads 中选出 M 大的子集，我们只介绍他们的打分函数。  
% 和 PAS 一样，这些打分函数也只能被允许使用部分特征。  

% - TEN：如之前所写，TEN 的 rank score 就是 tilde ctr * bid
% - REGCTR：使用 ctr 作为标签，用户和广告的部分特征作为特征，训练回归模型，loss 是 MSE。这似乎很像使用精细模型蒸馏得到一个粗糙的模型，但注意在这个场景中两个模型还有不同的特征。
% - REG：使用 ctr * bid 作为标签，用户和广告的部分特征作为特征，训练回归模型，loss 是 MSE。

% REGCTR 和 REG 和 PAS 的神经网络有相同的结构和输入，除了 REGCTR 不输入 bid 以外。
% 同时，REGCTR，REG 和 PAS 都直接或者间接的使用精细预估器的 ctr。
% 因此 regctr，reg, pas 主要的不同过就是损失函数。
% 我们引入 REGCTR 和 REG 方法的原因是为了体现 PAS 的损失函数针对预拍卖的问题是最为合理的。

To prove the effectiveness of our proposed solution PAS for pre-auction, we introduce following design of pre-auction for comparison. 
As all the methods work in a fashion of \emph{ranking by scores and truncating} to select a subset of $M$ ads from the all $N$ candidate ads, we mainly describe their rank score functions. 
These score functions are also restricted to use the same partial user and ad features as PAS uses.
The reason we introduce REGCTR and REG for comparison is to demonstrate that PAS's loss function is more proper for the problem of pre-auction.

\begin{itemize}
\item Tentative (TEN): As we described in previous section, the rank score of TEN for ad $i$ is simply $b_i\cdot \widetilde{ctr}_i$ where $\widetilde{ctr}$ is the output by the coarse estimator $\M^c$. 
\item Regression to $ctr_i$ (REGCTR): We use $ctr_i$ as label, and use partial user and ad features $\tilde{u}$, $\tilde{a}_i$ to train a regression model with mean square loss. 
The rank score is bid times output of the regression network.
REGCTR seems similar to the common technique of \emph{distilling} the refined estimator to obtain a coarse estimator, but note that the refined and coarse estimator have different access to features in this scenario.
\item Regression to $b_i \cdot ctr_i$ (REG): We use $b_i\cdot ctr_i$ as label, and use the partial user, ad features and the bid, \ie $b_i,\tilde{u}, \tilde{a}_i$, to train a regression model with mean square loss.  
\begin{comment}
% \item List-wise learning to rank (LTR): This method is from a supervised learning area called learning to rank (LTR) \cite{liu2011learning}, which studies mapping features from all set elements into a space of permutations. 
% We use the rank of the $N$ ads by $b\cdot ctr$ as label, and the common used practical loss function \emph{softmax cross entropy loss} \cite{cao2007learning}.
% \begin{equation*}
% % \label{eq:listnet-loss}
% \quad\quad L^{\mathcal{D}}_f = - \frac{1}{|\mathcal{D}|} \sum_{(x,y)} \sum_{i=1}^N \frac{\exp(y_i)}{\sum_{j=1}^N \exp(y_j)} \log \frac{\exp(f_i(x))}{\sum_{j=1}^N \exp(f_j(x))},
% \end{equation*}
% to train the score function. 
\end{comment}
\end{itemize}

The neural network structure and input for REGCTR, REG, and PAS are almost the same, except that REGCTR does not input bid.
Also, REGCTR, REG, PAS are all trained directly or indirectly with $ctr$ label from the refined estimator.
Therefore, the only major difference between these three methods is the loss function.

\begin{comment}
% We also compare the performance of with set encodings and without set encodings. 
% The methods without set encodings associated with PAS, REG, LTR are denoted as PASwoS, REGwoS, and LTRwoS, respectively. 
\end{comment}

\subsection{Evaluation Metrics}

We consider the following common used metrics for ad auction evaluation in our experiments. 
$\setA_N^K$ is the true top $K$ ads in the whole set $\setA_N$ while $\setA_M^K$ states the top $K$ ads in the selected set $\setA_M$ by pre-auction stage.  
\begin{itemize}
\item Social welfare rate: $SWr@K=\frac{\sum_{i\in \setA_M^K}b_i \cdot ctr_i}{\sum_{j\in \setA_N^K} b_j \cdot ctr_j}$.
\item Top K Recall: $Recall@K={\sum_{i\in \setA_M^K}\mathbf{1}[i\in \setA_N^K]} / K$.
%\item CTR rate: $CTRr=\frac{ \sum_{i=1\in\setA_M^K} ctr_i }{ \sum_{i=j\in\sx_N^K} ctr_j }$.
\item Revenue rate: $REVr@K=REV(\setA_M^K)/REV(\setA_N^K)$, where revenue $REV$ is under GSP auction and the subscript $(i)$ means the bidder with the $i$-th highest value of $b \cdot ctr$.
$$REV(\setA)=\sum_{i=1}^K b_{(i+1)}\cdot ctr_{(i+1)}.$$
\end{itemize}
Recall that we assume the bidders in this online advertising system are value maximizers, and under this assumption, GSP auction satisfies IC and IR. 
Therefore, we can regard the bid logged in this system which runs GSP mechanism is stable as it truthfully reflects the bidder's stable truthful value for a user click in recent period. 
Then, we can use the logged bid to compute social welfare and revenue while simulating other auction mechanisms which also satisfies IC and IR. 


\subsection{Performance Comparison}

% 针对 Public-1, Public-5 和 Industrial 三种数据设定的不同方法的结果分别在 Table 1 Table 2 Table 3 中。
% 表格中的结果展示了 均值、标准差和相对于 TEN 的提升，在每种数据设定和方法上的不同随机种子的 5 次实验。

Results of different methods on data setting Public-1, Public-5 and Industrial are given in Table.\ref{tab:perf-pub-01}, Table.\ref{tab:perf-pub-05} and Table.\ref{tab:perf-ind}, respectively.
These tables show average metrics, standard deviation and the improvement over baseline TEN in 5 runs with different random seeds for each data setting and methods.

% 首先，PAS 在所有的数据设定和方法中，相对于 TEN ，REGCTR，REG 都有非常显著的优势。
% 第二，REGCTR，REG，PAS 在绝大多数数据设定和指标上都相对于 TEN 有明显的提升。
% 说明引入第二阶段拍卖的信息来监督到预拍卖的训练是合理的。
% 第三，尽管 REGCTR 和 REG 在绝大多数数据设定和指标上都能够相对于 TEN 有明显提升，但是远远比不上 PAS。
% 说明 PAS 根据概率建模得到的学习 Top $K$ 概率的优化方法，相对于 REGCTR 和 REG 去回归第二阶段拍卖的 $ctr$ 或 $b_i\cdot ctr$ 的目标，更加适合预拍卖问题的集合选择的本质。
% 第四，大多数指标上 REG 相对于 REGCTR 有微弱的优势，说明回归中将 bid 引入特征和目标有正面的效果的，但是作用并不明显。

First, it is easy to see that our proposed PAS significantly outperforms all other methods in all data setting and all metrics. 
Second, as REGCTR, REG and PAS have better performance than TEN on most data settings and metrics, we can conclude that use the information from the second auction stage to supervise the pre-auction stage is reasonable.
Third, although REGCTR and REG achieve better results on most data setting and metrics, they still obliviously fall behind our proposed PAS. 
The reason can be interpreted as that while REGCTR and REG are forced to learn point-wise $ctr_i$ or $b_i\cdot ctr_i$, our proposed PAS, who models the probability for each ad to be top $K$, is a more proper evaluation metrics for the pre-auction stage. 
Fourth, REG weakly outperforms REGCTR in most cases. 
This can be interpreted as that introduce bid into feature and label has some positive effect for pre-auction method based on regression. 

% 下面，我们聚焦于 Public-1 和 Public-5 两个数据设定。
% Public-1 的降负采样率 < Public-5，从而导致粗糙 ctr 和 精细 ctr 之间的差距更大。
% 于是我们可以看到 TEN 在 Public-1 的绝大多数指标更差，同时 REGCTR 和 REG 的效果要差很多。
% REGCTR 和 REG 更适合精细 ctr 的方差更小的情况。
% 而 PAS 在两种设定下都有稳定的效果。

Next, we focus on the two data settings, Public-1 and Public-5, where all the features are the same while only the down negative sampling rates differ. 
Public-1 has a lower down negative sampling rate than Public-5, hence TEN on Public-1 has a worse performance than on Public-5 due to the larger gap coarse $\widetilde{ctr}$ and $ctr$. 
Also, both REGCTR and REG achieve a much worse performance on Public-1 than on Public-5.
This means that REGCTR and REG are more proper for data setting like Public-5, where the variance among $ctr$ and $b\cdot ctr$ in an auction are smaller, but not proper for the contrary setting like Public-1.
Moreover, we can see that our purposed PAS has stable good results in both data settings.

% 另外，比较不同的指标上的效果。我们发现 Recall 1 > recall 5 > recall 10 同时造成各自的提升呈现 recall 1 < recall 5 < recall 10。
% recall 的值比 sw 和 rev 要小，但是 recall 的增长明显比 social welfare 和 revenue 明显要大，这反映出了指标并不是完全一致。
% 但是，我们对于 PAS 的设计由于能够大幅提升 recall，所以能够大幅提升 sw 和 rev。

About different metrics, we see that recall@1 > recall@5 > recall@10, while the improvements on them are with contrary order. 
The absolute values of recall are less than social welfare rates and revenue rates, but the improvements on recall are more significant than those on social welfare rates and revenue rates. 
This means that $Recall@K$ is not completely the same as $SWr@K$ and $REVr@K$. 
However, as our design of PAS can improve $Recall@K$ much, the $SWr@K$ and $REVr@K$ also improve significantly. 

In Figure.\ref{fig:session-plot}, we plot an auction for each of the three data settings to demonstrate how different methods work in two-stage auction.

\subsection{IC Testing}

% 前面我们提到了要保证 IC IR 需要分配是关于 bid 单调的。  
% 因此我们需要 pre-auction 对于任意的广告主 i，满足给定了固定的广告特征和用户特征，以及其他广告的 bid 之后，广告主 i 进入 auction 的概率是关于 bid 单增。  
% 为了展示 PAS 的神经网络的实现能够近似实现上面提到的 pre-auction 的近似单调性，我们对于记录数据进行了反事实的扰动实验。这个实验同样在广告拍卖机制的激励兼容测试中用到。

As we have mentioned before that in order to guarantee the economics properties of IC and IR for the auction system, we require the allocation for each advertiser is monotonely increasing according to her bid. 
Therefore, we need the pre-auction stage to satisfy that for any advertiser $i$, given partial features for all ads $\bs{\tilde{a}}$ and the user features $\tilde{u}$, as well as bids from other advertisers $b_{-i}$, advertiser $i$ increases her probability of entering the auction stage when she increases bid $b_i$. 
To illustrate that neural networks for PAS can implement approximate monotone pre-auction, we conduct counter factual perturbation on each advertiser's bid in the logged data, which is also used in incentive property testing for ad auction mechanisms \cite{deng2019testing,deng2020data}.

% 具体的，我们从测试集中采样 1000 场拍卖。
% 定义一次测试为：固定一场拍卖中的一个广告。
% 对广告 i 进行测试时，网络的所有输入特征都不变，除了把 b_i 替换为 alpha * b_i，其中 alpha 是 [0.2, 2.0] 之间的一个乘性扰动因子。
% 这场拍卖的其他广告的特征全部不变。
% 接下来，我们模拟两阶段拍卖在这 10 个扰动因子上面的两阶段拍卖结果，看 PAS 网络是否通过测试
% 即，（1）存在一个扰动因子 underline alpha，当使用它或者更高的因子时，ad i 可以进入第二阶段；
% 或者（2）对于所有的 alpha，ad i 都无法进入第二阶段。

Specifically, we sample 1,000 auctions from the test dataset. 
One test is defined on an auction and an ad.
For an ad $i$ in test, all its features to PAS network remains the same except that we replace $b_i$ of ad $i$ with $\alpha\cdot bid_i$ where $\alpha\in \mathcal{S}_p=\{0.2 \times j|j=1,\ldots,10\}$ is a multiplicative perturbation factor from $[0.2, 2.0]$. 
All the features of other ads in this auction remains the same. 
Next, we simulate the two-stage auction on all 10 multiplicative perturbation factors to see if the PAS neural network fails in perturbation test, \ie (1) $\exists \underline{\alpha}\in \mathcal{S}_p$ such that $\forall \alpha \geq \underline{\alpha}$, ad $i$ can enter the auction stage with $\alpha\cdot b_i$; or (2) ad $i$ can not enter auction stage with $\alpha\cdot b_i$ for any $\alpha\in \mathcal{S}_p$. 

% 在 Public-1 和 Public-5 中，我们进行了 1000 * 1000 次测试，而在 Industrial 中，我们进行了 1000 * 700 次测试。
% 所有的方法在五次运行的均值和标准差展示在 表格 ic-pass 中，表格数值的单位是 10^{-5}。
% 我们看到对于 PAS 而言，测试失败率非常低。
% 即使我们没有在网络结构的设计中强行要求打分关于 bid 单调，网络也能够自动满足分配关于 bid 单调。
% 直觉上，这是因为我们的监督信号里面 bid 总是起到正向的作用。
% 我们同样对于 REG 进行了扰动测试，测试失败率也非常低。
% 表格中 TEN 和 REGCTR 因为都是采用最后单独乘 bid，所以本来 score 本来就满足对于 bid 单调，从而分配关于 bid 单调。

We conduct $1000\times 1000$ tests in each on Public-1 and Public-5; and in Industrial, we conduct $1000\times 700$ tests. 
The average results and standard deviation of 5 runs are listed in Table.\ref{tab:ic-pass}, where the unit of values is $\times 10^{-5}$.
The very low failure rate in the perturbation tests shows that even we apply no deliberate design on PAS neural networks for a guarantee of strictly non-decreasing allocation according to bid, the learning based methods satisfy monotonicity to some extend automatically. 
Intuitively, this is due to that there is a signal from the supervised data that bid has a positive effect on the optimization objective. 
We also test REG networks, and also obtain similarly very low failure rate as PAS.
For TEN and REGCTR, as they only time bid with the $\widetilde{ctr}$ or regression of $ctr$, the corresponding scores and hence the allocation of pre-auction, are monotone according to bid. 

\input{21fupa_main_wsdm/21fupa_tab_ic_test.tex}

% ====

==> 21fupa_main_wsdm/fig/21fupa_related.tex <==
\section{Related Work}

\textbf{Online advertising auction.} 
This work is motivated from the market of online advertising auction, where traditional auction mechanisms like general second price auction (GSP)~\cite{edelman2007internet,varian2007position} and Vickrey-Clark-Groove auction (VCG)~\cite{varian2014vcg} are widely used.
Recently, many parametric mechanisms learning from data are proposed to optimize performance metrics of the auction market, \eg squashed GSP~\cite{lahaie2007revenue}, boosted second price auction~\cite{golrezaei2017boosted}, and dynamic reserve price via reinforcement learning~\cite{shen2020reinforcement} for the task of revenue maximization. The paradigm of differentiable mechanism design via deep learning proposed by D{\"u}tting \etal~\cite{dutting2019optimal} is also applied to multi-objective optimization in online advertising auctions~\cite{liu2021neural}.

\textbf{Two-stage recommenders.} 
Two-stage architectures with candidate generation followed by ranking have been widely adopted in large scale industrial recommenders. 
Despite their popularity, the literature on two-stage recommenders is relatively scarce. 
To improve computation efficiency \cite{kang2019candidate,yi2019sampling} and recommendation quality \cite{chen2019top} are still the two most important problems even in two-stage settings. 
Interaction between the two stages and its influence on system performance are studied in \cite{chen2019top,ma2020off,hron2020exploration}. 
Our problem of two-stage auction system differs from the two-stage recommenders because we need quantifiable evaluation of user's interests, \eg $ctr$ along as advertisers' bids to determine both allocation and payment while the recommender only determines the order of items and no payment. Furthermore, auction system are required to satisfy desired economics properties. 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)
